Cube2Pipes : Investigating Hybrid Gameplay Using AR and a Tangible 3D Puzzle

We present our game, Cube2Pipes, as an attempt to investigate a unique gameplay design where we use a tangible 3D spatial puzzle, in the form of a 2X2 Rubik's Cube, as an interface to a tabletop mobile augmented reality (AR) game. The game interface adapts to user movement and interaction with both virtual and tangible elements via computer vision based tracking. This game can be seen as an instance of generic interactive hybrid systems as it involves interaction with both virtual and real, tangible elements. We present a thorough user evaluation about various aspects of the gameplay in order to answer the question as to whether hybrid gameplay involving both real and virtual interfaces and elements is more captivating and preferred by users, than standard (baseline) gameplay with only virtual elements. We use multiple industry standard user study questionnaires to try and answer this question. We also try to determine whether the game facilitates understanding of the spatial moves required to solve a Rubik's Cube, and the efficacy of a tangible puzzle interface to a tabletop AR game.

==> 032virtualTerrain.tex <==
\subsection{Virtual Terrain}\label{virTer}
The virtual terrain surface is created by changing the elevation of rectangular grid cells. The grid is overlaid on any flat surface  on which the game board marker is placed (see Figure~\ref{figgameMarker_a}). Additionally, the terrain consists of static assets including a long river, a water tank, a shop and three houses. 
%The water tank is placed at top of the highest elevated grid of the terrain, and the river is placed on a contiguous set of grid cells such that the shop and rest of the terrain is separated by the river. Some assets, like the houses, are randomly placed at the remaining non-elevated and unoccupied grids. 

The player is represented by a virtual character in the scene. The movement of this virtual character is controlled by the player using a joystick button on the mobile screen. 
The assets that are acquired by the user during gameplay are called dynamic assets. 
Their usage is controlled by the player. 
The goal of the game is to lay fixed length horizontal/vertical pipes, with different decrements in pressure, between the water tank and the houses while maintaining the minimum required water pressure in the pipes.
%The pipes have to be acquired from the shop using money and keys gathered during the game. Water pressure falls along the length of the pipeline. 
%Four different pipes of fixed length with different decrements in water pressure (indicating different pipe diameters) are provided. Pipes of both horizontal or vertical orientations are available. 
The vertical pipes are used to lay pipe between elevated and non-elevated grid cells. These are laid inside the raised terrain and are often not very visible on the screen. Horizontal pipes can be used to lay pipe between two grid cells at the same height. The player needs to mix and match different combinations of these pipes to complete the task. Along with the pipes, three other assets, namely fences, ladders and bridges, can also be placed in the scene by the player. The ladders are used to climb up and down from the elevated grid cells. Bridges are used to cross the river. The fence has to be used to create a boundary around the water tank by the player. Another asset, called the time asset, can be used by the player for some pre-defined number of times to boost up the water pressure in the pipeline like a pump. This is helpful when the water pressure falls below the minimum pressure. Once acquired, all assets can be viewed by using the view inventory buttons.
The player wins the game when all the houses are connected through pipes with the water tank while the minimum water pressure through the pipes is maintained.
The game is lost whenever the water pressure in the pipe drops below the minimum value. 
Figure~\ref{figterrainAssets_b} shows all the dynamic assets of the game. In the next subsection, we describe the mechanism to gather these assets to play the game.
Figure~\ref{figterrainGoAround} shows how various new game elements or assets can be revealed on the screen as the user walks around the area of augmentation while pointing the mobile device at it. 
%This helps the user to get a different view of the virtual 3D terrain. 
This is possible only because of the AR aspect of the terrain display and it makes the game more believable for the user. It also helps the user to place various dynamic assets conveniently on the 3D terrain, while viewing it from different locations around the physical plane on which the terrain is displayed. 
\begin{figure}[h!t]
    \centering
    \subfloat{\includegraphics[width=0.45\columnwidth]{pictures/terrain_view_01.pdf}}~~
    \subfloat{\includegraphics[width=0.45\columnwidth]{pictures/terrain_view_02.pdf}}
    \caption{The terrain viewed from different viewpoints can reveal new elements or assets in the game.}
    \label{figterrainGoAround}
\end{figure}


==> 033augmentedCube.tex <==
\subsection{Augmented Cube}\label{augCube}
As mentioned in the beginning of the section, the dynamic assets required for playing the game have to gathered by solving a $2\times2$ Rubik's Cube.  
A \textit{magical} portal (see Figure~\ref{figterrainAssets_a}), to transport the virtual boy on the top of a cell of the cube, appears on the virtual terrain at different points of time during the game till the cube is solved.
%where the player needs to make the required rotations of the cube to gather particular assets. 
This allows for seamless gameplay between the terrain and the challenge puzzle. The solution of the cube is check-pointed by two stages - solving the bottom face and bottom layers of all other faces except the top face, and solving the remaining of the cube (see Figure~\ref{figcubeNot} for visual description of the layers and the faces of a cube). 
\begin{figure}[h!tb]
    \centering
    \subfloat[Cell, layer and face of a Rubik's Cube.\label{figcubeNot}]
    {\includegraphics[width=0.29\columnwidth]{pictures/cube_notation.pdf}}~~~~
    \subfloat[Visual cue for rotating a layer.\label{figaugCube_a}]{\includegraphics[width=0.30\columnwidth]{pictures/cube_layer_rotation.pdf}}~~
    \subfloat[Visual cue for turning the cube.\label{figaugCube_b}]{\includegraphics[width=0.30\columnwidth]{pictures/cube_face_rotation.pdf}}
    \caption{Parts of a Rubik's cube and augmented visual cues.}
\end{figure}
The markers shown in Figure~\ref{figgameMarker_b} are pasted on each cell of the cube and are used to track them.  The markers are arranged on the cube such that on solving it, all the markers representing the same asset (ladders, bridges, clocks, bags of money, keys and fences) appear on the same face. The "shuffling" or "rotation" of the cube serves as the basic movement for initiating any action. Augmented visual cues in form of the virtual character, a 3D target asset and a directed arrows are provided for assistance in solving the cube. The virtual character and the target asset(bag of money) are placed on two cells representing a rotation in the direction from the character to the target asset. This cue corresponds to rotating the layer of the cube which contains these two cells. If instead of a layer, the entire cube needs to be rotated, an arrow is shown at the centre of the cube to represent turning the entire cube in direction of the arrow. 
Figure~\ref{figaugCube_a} and~\ref{figaugCube_b} shows the two kinds of augmentations on the cube. The augmentations changes dynamically after each rotation made by the player to represent the next required step from the series of computed steps to solve the cube.

At each check-point of cube solution, the virtual character is transported back to the virtual terrain. At this stage, the assets corresponding to the cells at correct positions in the cube can be used for navigating the terrain. 
 %After the first checkpoint, the assets corresponding to the markers at the bottom face and bottom layers of all other faces except the top face can be used by the player. After the second checkpoint, all the assets, if not already used up, are accessible to the player. 
As the game engine guides the player about the next required step, it can also detect an incorrect step up to one rotation in any direction made by her and change the next required steps accordingly.
This makes the cube solver and the augmentations robust to some player error. 
Multiple incorrect steps, that is multiple incorrect rotations to the cube, leads to losing the game.

==> 034implementation.tex <==
\subsection{Implementation \label{implMet}}
The game is implemented using the Google ARCore SDK~\cite{arcore}, Unity 3D~\cite{unity} and Blender~\cite{blender}.  See Supplementary materials for more details. The minimum requirement for accessing the game is an ARCore enabled smartphone, a $2 \times 2$ Rubik's cube and the set of markers.

==> 06conclusion.tex <==
\section{Conclusion}\label{conclu}
We design and present an interactive, AR based hybrid game called \textit{Cube2Pipes}. The gameplay is a unique combination of a virtual tabletop game and a tangible challenge puzzle interface of a $2\times2$ Rubik's Cube. A thorough user evaluation of the complete game is done using well established methods. 
The use of the tangible component in the hybrid game makes it interesting as per SUS scores. The workload on the user does not increase much with the extra level of challenge by adding Rubik's Cube solution to the pipe laying problem as per NASA TLX score. The addition of solving Rubik's Cube to the game does not add to the effort of playing the game while maintaining a degree of involvement with the interface as per the Presence evaluation. Also, the visual augmented cues based method of solving the Rubik's Cube independently has a good Presence score, which is congruent with the results of solution method comparison study.

We are thus able to conclusively infer that such a hybrid game is quite believable and engaging for the user. As an add-on advantage of this gaming mechanism, the user is also able to learn the spatial moves required to solve the Rubik's Cube in an organic way. 

A limitation of our game is the quality of graphics. The visual design of the assets and the movement animation of the character in the game should be improved. Though if the users find the gameplay interesting enough, they do not complain about the graphics. A major implementation challenge is to resolve the various lags and delays that occur due to a prolonged usage of the AR platform or quickly changing image markers. We want to extend the challenge mechanism to a $3\times3$ Rubik's Cube, however, the degrees of freedom of the solution space for the cube makes it a very tricky problem to solve.



==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

